Reinforcement Learning for IoT Security: A Comprehensive Survey

The number of connected smart devices has been increasing exponentially for different Internet-of-Things (IoT) applications. Security has been a long run challenge in the IoT systems which has many attack vectors, security flaws and vulnerabilities. Securing billions of B connected devices in IoT is a must task to realize the full potential of IoT applications. Recently, researchers have proposed many security solutions for IoT. Machine learning has been proposed as one of the emerging solutions for IoT security and Reinforcement learning is gaining more popularity for securing IoT systems. Reinforcement learning, unlike other machine learning techniques, can learn the environment by having minimum information about the parameters to be learned. It solves the optimization problem by interacting with the environment adapting the parameters on the fly. In this paper, we present an comprehensive survey of different types of cyber-attacks against different IoT systems and then we present reinforcement learning and deep reinforcement learning based security solutions to combat those different types of attacks in different IoT systems. Furthermore, we present the Reinforcement learning for securing CPS systems (i.e., IoT with feedback and control) such as smart grid and smart transportation system. The recent important attacks and countermeasures using reinforcement learning B in IoT are also summarized in the form of tables. With this paper, readers can have a more thorough understanding of IoT security attacks and countermeasures using Reinforcement Learning, as well as research trends in this area.

==> references_CPS.tex <==
@article{atzori2010internet,
  title={The internet of things: A survey},
  author={Atzori, Luigi and Iera, Antonio and Morabito, Giacomo},
  journal={Computer networks},
  volume={54},
  number={15},
  pages={2787--2805},
  year={2010},
  publisher={Elsevier}
}

@article{mansfield2018open,
	title={Open source and the Internet of Things},
	author={Mansfield-Devine, Steve},
	journal={Network Security},
	volume={2018},
	number={2},
	pages={14--19},
	year={2018},
	publisher={Elsevier}
}

@article{min2018learning,
	title={{Learning-based privacy-aware offloading for healthcare IoT with energy harvesting}},
	author={Min, Minghui and Wan, Xiaoyue and Xiao, Liang and Chen, Ye and Xia, Minghua and Wu, Di and Dai, Huaiyu},
	journal={IEEE Internet of Things Journal},
	volume={6},
	number={3},
	pages={4307--4316},
	year={2018}
}


@article{rawat2018performance,
	title={{On the performance of cognitive internet-of-vehicles with unlicensed user-mobility and licensed user-activity}},
	author={Rawat, Danda B and Alsabet, Reham and Bajracharya, Chandra and Song, Min},
	journal={Computer Networks},
	volume={137},
	pages={98--106},
	year={2018},
	publisher={Elsevier}
}


@techreport{rawat2017vehicular,
	title={{Vehicular Cyber Physical Systems: Adaptive Connectivity and Security}},
	author={Rawat, Danda B and Bajracharya, Chandra},
	year={2017},
	institution={Springer}
}

@article{felix2020sur,
	title={{Resilient Machine Learning for Networked Cyber Physical Systems: A Survey for Machine Learning Security to Securing Machine Learning for CPS}},
	author={Felix Olowononi and Danda B. Rawat and Chunmei Liu},
	journal={IEEE Communications Surveys and Tutorials},
	year={2020},
	note  = {Early Access, DoI: https://doi.org/10.1109/COMST.2020.3036778}
}
 

 @article{caminero2019adversarial,
 	title={Adversarial environment reinforcement learning algorithm for intrusion detection},
 	author={Caminero, Guillermo and Lopez-Martin, Manuel and Carro, Belen},
 	journal={Computer Networks},
 	volume={159},
 	pages={96--109},
 	year={2019},
 	publisher={Elsevier}
 }

@book{sutton2018reinforcement,
	title={Reinforcement learning: An introduction},
	author={Sutton, Richard S and Barto, Andrew G},
	year={2018},
	publisher={MIT press}
}


@ARTICLE{5227780, author={F. L. {Lewis} and D. {Vrabie}}, journal={IEEE Circuits and Systems Magazine}, title={Reinforcement learning and adaptive dynamic programming for feedback control}, year={2009}, volume={9}, number={3}, pages={32-50},}

@article{barto2003recent,
	title={Recent advances in hierarchical reinforcement learning},
	author={Barto, Andrew G and Mahadevan, Sridhar},
	journal={Discrete event dynamic systems},
	volume={13},
	number={1-2},
	pages={41--77},
	year={2003},
	publisher={Springer}
}


@article{schultz1997neural,
	title={A neural substrate of prediction and reward},
	author={Schultz, Wolfram and Dayan, Peter and Montague, P Read},
	journal={Science},
	volume={275},
	number={5306},
	pages={1593--1599},
	year={1997},
	publisher={American Association for the Advancement of Science}
}

@article{hinton2006reducing,
	title={Reducing the dimensionality of data with neural networks},
	author={Hinton, Geoffrey E and Salakhutdinov, Ruslan R},
	journal={science},
	volume={313},
	number={5786},
	pages={504--507},
	year={2006},
	publisher={American Association for the Advancement of Science}
}

@INPROCEEDINGS{8260800, author={I. {Kachalsky} and I. {Zakirzyanov} and V. {Ulyantsev}}, booktitle={2017 16th IEEE International Conference on Machine Learning and Applications (ICMLA)}, title={Applying Reinforcement Learning and Supervised Learning Techniques to Play Hearthstone}, year={2017}, volume={}, number={}, pages={1145-1148},}


@inproceedings{mnih2016asynchronous,
	title={Asynchronous methods for deep reinforcement learning},
	author={Mnih, Volodymyr and Badia, Adria Puigdomenech and Mirza, Mehdi and Graves, Alex and Lillicrap, Timothy and Harley, Tim and Silver, David and Kavukcuoglu, Koray},
	booktitle={International conference on machine learning},
	pages={1928--1937},
	year={2016}
}

@book{weber2008reinforcement,
	title={Reinforcement Learning},
	author={Weber, Cornelius and Elshaw, Mark and Mayer, N Michael},
	year={2008},
	publisher={BoD--Books on Demand}
}

@article{franccois2018introduction,
	title={An introduction to deep reinforcement learning},
	author={Fran{\c{c}}ois-Lavet, Vincent and Henderson, Peter and Islam, Riashat and Bellemare, Marc G and Pineau, Joelle and others},
	journal={Foundations and Trends{\textregistered} in Machine Learning},
	volume={11},
	number={3-4},
	pages={219--354},
	year={2018},
	publisher={Now Publishers, Inc.}
}

@INPROCEEDINGS{7983780, author={S. P. K. {Spielberg} and R. B. {Gopaluni} and P. D. {Loewen}}, booktitle={2017 6th International Symposium on Advanced Control of Industrial Processes (AdCONIP)}, title={Deep reinforcement learning approaches for process control}, year={2017}, volume={}, number={}, pages={201-206},}


@inproceedings{mao2016resource,
	title={Resource management with deep reinforcement learning},
	author={Mao, Hongzi and Alizadeh, Mohammad and Menache, Ishai and Kandula, Srikanth},
	booktitle={Proceedings of the 15th ACM Workshop on Hot Topics in Networks},
	pages={50--56},
	year={2016}
}

@article{zhang2017intelligent,
	title={Intelligent cloud resource management with deep reinforcement learning},
	author={Zhang, Yu and Yao, Jianguo and Guan, Haibing},
	journal={IEEE Cloud Computing},
	volume={4},
	number={6},
	pages={60--69},
	year={2017},
	publisher={IEEE}
}

@article{vecerik2017leveraging,
	title={Leveraging demonstrations for deep reinforcement learning on robotics problems with sparse rewards},
	author={Vecerik, Mel and Hester, Todd and Scholz, Jonathan and Wang, Fumin and Pietquin, Olivier and Piot, Bilal and Heess, Nicolas and Roth{\"o}rl, Thomas and Lampe, Thomas and Riedmiller, Martin},
	journal={arXiv preprint arXiv:1707.08817},
	year={2017}
}
@inproceedings{gu2017deep,
	title={Deep reinforcement learning for robotic manipulation with asynchronous off-policy updates},
	author={Gu, Shixiang and Holly, Ethan and Lillicrap, Timothy and Levine, Sergey},
	booktitle={2017 IEEE international conference on robotics and automation (ICRA)},
	pages={3389--3396},
	year={2017},
	organization={IEEE}
}

@article{wang2016survey,
	title={A survey on applications of model-free strategy learning in cognitive wireless networks},
	author={Wang, Wenbo and Kwasinski, Andres and Niyato, Dusit and Han, Zhu},
	journal={IEEE Communications Surveys \& Tutorials},
	volume={18},
	number={3},
	pages={1717--1757},
	year={2016},
	publisher={IEEE}
}

@article{ling2015application,
	title={Application of reinforcement learning for security enhancement in cognitive radio networks},
	author={Ling, Mee Hong and Yau, Kok-Lim Alvin and Qadir, Junaid and Poh, Geong Sen and Ni, Qiang},
	journal={Applied Soft Computing},
	volume={37},
	pages={809--829},
	year={2015},
	publisher={Elsevier}
}

@article{wang2019survey,
	title={A survey of dynamic spectrum allocation based on reinforcement learning algorithms in cognitive radio networks},
	author={Wang, Yonghua and Ye, Zifeng and Wan, Pin and Zhao, Jiajun},
	journal={Artificial Intelligence Review},
	volume={51},
	number={3},
	pages={493--506},
	year={2019},
	publisher={Springer}
}

@article{garcia2009anomaly,
	title={Anomaly-based network intrusion detection: Techniques, systems and challenges},
	author={Garcia-Teodoro, Pedro and Diaz-Verdejo, Jesus and Maci{\'a}-Fern{\'a}ndez, Gabriel and V{\'a}zquez, Enrique},
	journal={computers \& security},
	volume={28},
	number={1-2},
	pages={18--28},
	year={2009},
	publisher={Elsevier}
}

@book{dua2016data,
	title={Data mining and machine learning in cybersecurity},
	author={Dua, Sumeet and Du, Xian},
	year={2016},
	publisher={CRC press}
}

@article{buczak2015survey,
	title={A survey of data mining and machine learning methods for cyber security intrusion detection},
	author={Buczak, Anna L and Guven, Erhan},
	journal={IEEE Communications surveys \& tutorials},
	volume={18},
	number={2},
	pages={1153--1176},
	year={2015},
	publisher={IEEE}
}

@article{berman2019survey,
	title={A survey of deep learning methods for cyber security},
	author={Berman, Daniel S and Buczak, Anna L and Chavis, Jeffrey S and Corbett, Cherita L},
	journal={Information},
	volume={10},
	number={4},
	pages={122},
	year={2019},
	publisher={Multidisciplinary Digital Publishing Institute}
}

@article{biswas2018intrusion,
	title={Intrusion detection using machine learning: A comparison study},
	author={Biswas, Saroj Kr},
	journal={International Journal of Pure and Applied Mathematics},
	volume={118},
	number={19},
	pages={101--114},
	year={2018}
}

@article{xin2018machine,
	title={Machine learning and deep learning methods for cybersecurity},
	author={Xin, Yang and Kong, Lingshuang and Liu, Zhi and Chen, Yuling and Li, Yanmiao and Zhu, Hongliang and Gao, Mingcheng and Hou, Haixia and Wang, Chunhua},
	journal={IEEE Access},
	volume={6},
	pages={35365--35381},
	year={2018},
	publisher={IEEE}
}

@article{milosevic2017machine,
	title={Machine learning aided Android malware classification},
	author={Milosevic, Nikola and Dehghantanha, Ali and Choo, Kim-Kwang Raymond},
	journal={Computers \& Electrical Engineering},
	volume={61},
	pages={266--274},
	year={2017},
	publisher={Elsevier}
}

@article{kp2018short,
	title={A short review on Applications of Deep learning for Cyber security},
	author={KP, Soman and others},
	journal={arXiv preprint arXiv:1812.06292},
	year={2018}
}

@article{rege2018machine,
	title={Machine learning for cyber defense and attack},
	author={Rege, Manjeet and Mbah, Raymond Blanch K},
	journal={DATA ANALYTICS 2018},
	pages={83},
	year={2018}
}

@article{berman2019survey,
	title={A survey of deep learning methods for cyber security},
	author={Berman, Daniel S and Buczak, Anna L and Chavis, Jeffrey S and Corbett, Cherita L},
	journal={Information},
	volume={10},
	number={4},
	pages={122},
	year={2019},
	publisher={Multidisciplinary Digital Publishing Institute}
}

@article{ding2018survey,
	title={A survey on security control and attack detection for industrial cyber-physical systems},
	author={Ding, Derui and Han, Qing-Long and Xiang, Yang and Ge, Xiaohua and Zhang, Xian-Ming},
	journal={Neurocomputing},
	volume={275},
	pages={1674--1683},
	year={2018},
	publisher={Elsevier}
}

@article{wu2019detecting,
	title={Detecting cyber-physical attacks in CyberManufacturing systems with machine learning methods},
	author={Wu, Mingtao and Song, Zhengyi and Moon, Young B},
	journal={Journal of intelligent manufacturing},
	volume={30},
	number={3},
	pages={1111--1123},
	year={2019},
	publisher={Springer}
}

@article{xiao2018iot,
	title={IoT security techniques based on machine learning: How do IoT devices use AI to enhance security?},
	author={Xiao, Liang and Wan, Xiaoyue and Lu, Xiaozhen and Zhang, Yanyong and Wu, Di},
	journal={IEEE Signal Processing Magazine},
	volume={35},
	number={5},
	pages={41--49},
	year={2018},
	publisher={IEEE}
}

@article{nguyen2019deep,
	title={Deep Reinforcement Learning for Cyber Security},
	author={Nguyen, Thanh Thi and Reddi, Vijay Janapa},
	journal={arXiv preprint arXiv:1906.05799},
	year={2019}
}

@article{beard1997galerkin,
	title={Galerkin approximations of the generalized Hamilton-Jacobi-Bellman equation},
	author={Beard, Randal W and Saridis, George N and Wen, John T},
	journal={Automatica},
	volume={33},
	number={12},
	pages={2159--2177},
	year={1997},
	publisher={Elsevier}
}

@article{dreyfus2002richard,
	title={Richard Bellman on the birth of dynamic programming},
	author={Dreyfus, Stuart},
	journal={Operations Research},
	volume={50},
	number={1},
	pages={48--51},
	year={2002},
	publisher={INFORMS}
}

@article{mnih2013playing,
	title={Playing atari with deep reinforcement learning},
	author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Graves, Alex and Antonoglou, Ioannis and Wierstra, Daan and Riedmiller, Martin},
	journal={arXiv preprint arXiv:1312.5602},
	year={2013}
}

@article{silver2016mastering,
	title={Mastering the game of Go with deep neural networks and tree search},
	author={Silver, David and Huang, Aja and Maddison, Chris J and Guez, Arthur and Sifre, Laurent and Van Den Driessche, George and Schrittwieser, Julian and Antonoglou, Ioannis and Panneershelvam, Veda and Lanctot, Marc and others},
	journal={nature},
	volume={529},
	number={7587},
	pages={484},
	year={2016},
	publisher={Nature Publishing Group}
}

@article{mnih2015human,
	title={Human-level control through deep reinforcement learning},
	author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Rusu, Andrei A and Veness, Joel and Bellemare, Marc G and Graves, Alex and Riedmiller, Martin and Fidjeland, Andreas K and Ostrovski, Georg and others},
	journal={Nature},
	volume={518},
	number={7540},
	pages={529--533},
	year={2015},
	publisher={Nature Publishing Group}
}

@article{silver2017mastering,
	title={Mastering the game of go without human knowledge},
	author={Silver, David and Schrittwieser, Julian and Simonyan, Karen and Antonoglou, Ioannis and Huang, Aja and Guez, Arthur and Hubert, Thomas and Baker, Lucas and Lai, Matthew and Bolton, Adrian and others},
	journal={Nature},
	volume={550},
	number={7676},
	pages={354--359},
	year={2017},
	publisher={Nature Publishing Group}
}

@inproceedings{van2016deep,
	title={Deep reinforcement learning with double q-learning},
	author={Van Hasselt, Hado and Guez, Arthur and Silver, David},
	booktitle={Thirtieth AAAI conference on artificial intelligence},
	year={2016}
}

@article{wang2015dueling,
	title={Dueling network architectures for deep reinforcement learning},
	author={Wang, Ziyu and Schaul, Tom and Hessel, Matteo and Van Hasselt, Hado and Lanctot, Marc and De Freitas, Nando},
	journal={arXiv preprint arXiv:1511.06581},
	year={2015}
}

@article{lillicrap2015continuous,
	title={Continuous control with deep reinforcement learning},
	author={Lillicrap, Timothy P and Hunt, Jonathan J and Pritzel, Alexander and Heess, Nicolas and Erez, Tom and Tassa, Yuval and Silver, David and Wierstra, Daan},
	journal={arXiv preprint arXiv:1509.02971},
	year={2015}
}

@article{li2011smart,
	title={Smart community: an internet of things application},
	author={Li, Xu and Lu, Rongxing and Liang, Xiaohui and Shen, Xuemin and Chen, Jiming and Lin, Xiaodong},
	journal={IEEE Communications magazine},
	volume={49},
	number={11},
	pages={68--75},
	year={2011},
	publisher={IEEE}
}

@inproceedings{andrea2015internet,
	title={Internet of Things: Security vulnerabilities and challenges},
	author={Andrea, Ioannis and Chrysostomou, Chrysostomos and Hadjichristofi, George},
	booktitle={2015 IEEE Symposium on Computers and Communication (ISCC)},
	pages={180--187},
	year={2015},
	organization={IEEE}
}

@article{roman2013features,
	title={On the features and challenges of security and privacy in distributed internet of things},
	author={Roman, Rodrigo and Zhou, Jianying and Lopez, Javier},
	journal={Computer Networks},
	volume={57},
	number={10},
	pages={2266--2279},
	year={2013},
	publisher={Elsevier}
}

@article{alaba2017internet,
	title={Internet of Things security: A survey},
	author={Alaba, Fadele Ayotunde and Othman, Mazliza and Hashem, Ibrahim Abaker Targio and Alotaibi, Faiz},
	journal={Journal of Network and Computer Applications},
	volume={88},
	pages={10--28},
	year={2017},
	publisher={Elsevier}
}

@inproceedings{alanazi2015resilience,
	title={On resilience of Wireless Mesh routing protocol against DoS attacks in IoT-based ambient assisted living applications},
	author={Alanazi, Shaker and Al-Muhtadi, Jalal and Derhab, Abdelouahid and Saleem, Kashif and AlRomi, Afnan N and Alholaibah, Hanan S and Rodrigues, Joel JPC},
	booktitle={2015 17th International Conference on E-health Networking, Application \& Services (HealthCom)},
	pages={205--210},
	year={2015},
	organization={IEEE}
}

@article{malialis2015distributed,
	title={Distributed response to network intrusions using multiagent reinforcement learning},
	author={Malialis, Kleanthis and Kudenko, Daniel},
	journal={Engineering Applications of Artificial Intelligence},
	volume={41},
	pages={270--284},
	year={2015},
	publisher={Elsevier}
}

@article{yau2005defending,
	title={Defending against distributed denial-of-service attacks with max-min fair server-centric router throttles},
	author={Yau, David KY and Lui, John CS and Liang, Feng and Yam, Yeung},
	journal={IEEE/ACM Transactions on Networking},
	volume={13},
	number={1},
	pages={29--42},
	year={2005},
	publisher={IEEE}
}

@inbook{inbook,
	author = {Romdhani, Imed and Abdmeziem, Riad and Tandjaoui, D.},
	year = {2015},
	month = {07},
	pages = {},
	title = {Architecting the Internet of Things: State of the Art},
	isbn = {ISSN: 2198-4182}
}

@inproceedings{wu2010research,
	title={Research on the architecture of Internet of Things},
	author={Wu, Miao and Lu, Ting-Jie and Ling, Fei-Yang and Sun, Jing and Du, Hui-Ying},
	booktitle={2010 3rd International Conference on Advanced Computer Theory and Engineering (ICACTE)},
	volume={5},
	pages={V5--484},
	year={2010},
	organization={IEEE}
}

@article{wang2016internet,
	title={The Internet of Things: a security point of view},
	author={Wang, Pan and Chaudhry, Sohail and Li, Ling and Li, Shancang and Tryfonas, Theo and Li, Honglei},
	journal={Internet Research},
	year={2016},
	publisher={Emerald Group Publishing Limited}
}

@inproceedings{zhong2015study,
	title={Study on the IOT architecture and gateway technology},
	author={Zhong, Chang-Le and Zhu, Zhen and Huang, Ren-Gen},
	booktitle={2015 14th International Symposium on Distributed Computing and Applications for Business Engineering and Science (DCABES)},
	pages={196--199},
	year={2015},
	organization={IEEE}
}

@inproceedings{finkenzeller2009known,
	title={Known attacks on RFID systems, possible countermeasures and upcoming standardisation activities},
	author={Finkenzeller, Klaus},
	booktitle={5th European Workshop on RFID Systems and Technologies},
	pages={1--31},
	year={2009}
}

@article{mitrokotsa2010classification,
	title={Classification of RFID attacks},
	author={Mitrokotsa, Aikaterini and Rieback, Melanie R and Tanenbaum, Andrew S},
	journal={Gen},
	volume={15693},
	number={14443},
	pages={14},
	year={2010},
	publisher={Citeseer}
}

@article{chien2007security,
	title={Security of ultra-lightweight RFID authentication protocols and its improvements},
	author={Chien, Hung-Yu and Huang, Chen-Wei},
	journal={ACM SIGOPS Operating Systems Review},
	volume={41},
	number={4},
	pages={83--86},
	year={2007},
	publisher={ACM New York, NY, USA}
}

@inproceedings{deng2005defending,
	title={Defending against path-based DoS attacks in wireless sensor networks},
	author={Deng, Jing and Han, Richard and Mishra, Shivakant},
	booktitle={Proceedings of the 3rd ACM workshop on Security of ad hoc and sensor networks},
	pages={89--96},
	year={2005}
}

@article{sonar2014survey,
	title={A survey: DDOS attack on Internet of Things},
	author={Sonar, Krushang and Upadhyay, Hardik},
	journal={International Journal of Engineering Research and Development},
	volume={10},
	number={11},
	pages={58--63},
	year={2014}
}

@inproceedings{malialis2013multiagent,
	title={Multiagent router throttling: Decentralized coordinated response against ddos attacks},
	author={Malialis, Kleanthis and Kudenko, Daniel},
	booktitle={Twenty-Fifth IAAI Conference},
	year={2013}
}

@inproceedings{liu2018deep,
	title={Deep reinforcement learning based smart mitigation of DDoS flooding in software-defined networks},
	author={Liu, Yandong and Dong, Mianxiong and Ota, Kaoru and Li, Jianhua and Wu, Jun},
	booktitle={2018 IEEE 23rd International Workshop on Computer Aided Modeling and Design of Communication Links and Networks (CAMAD)},
	pages={1--6},
	year={2018},
	organization={IEEE}
}

@article{fang2013loss,
	title={A loss-free multipathing solution for data center network using software-defined networking approach},
	author={Fang, Shuo and Yu, Yang and Foh, Chuan Heng and Aung, Khin Mi Mi},
	journal={IEEE transactions on magnetics},
	volume={49},
	number={6},
	pages={2723--2730},
	year={2013},
	publisher={IEEE}
}

@article{hu2014survey,
	title={A survey on software-defined network and openflow: From concept to implementation},
	author={Hu, Fei and Hao, Qi and Bao, Ke},
	journal={IEEE Communications Surveys \& Tutorials},
	volume={16},
	number={4},
	pages={2181--2206},
	year={2014},
	publisher={IEEE}
}

@INPROCEEDINGS{8276173, author={D. G. {Bhoyar} and U. {Yadav}}, booktitle={2017 International Conference on Innovations in Information, Embedded and Communication Systems (ICIIECS)}, title={Review of jamming attack using game theory}, year={2017}, volume={}, number={}, pages={1-4},}

@article{grover2014jamming,
	title={Jamming and anti-jamming techniques in wireless networks: a survey},
	author={Grover, Kanika and Lim, Alvin and Yang, Qing},
	journal={International Journal of Ad Hoc and Ubiquitous Computing},
	volume={17},
	number={4},
	pages={197--215},
	year={2014},
	publisher={Inderscience Publishers, Geneva, SWITZERLAND}
}

@inproceedings{weber2010towards,
	title={Towards trustworthy identity and access management for the future internet},
	author={Weber, Stefan G and Martucci, Leonardo and Ries, Sebastian and M{\"u}hlh{\"a}user, Max},
	booktitle={4th International Workshop on Trustworthy Internet of People, Things \& Services},
	year={2010}
}


@INPROCEEDINGS{7841922, author={N. {Namvar} and W. {Saad} and N. {Bahadori} and B. {Kelley}}, booktitle={2016 IEEE Global Communications Conference (GLOBECOM)}, title={Jamming in the Internet of Things: A Game-Theoretic Perspective}, year={2016}, volume={}, number={}, pages={1-6},}

@article{wu2011anti,
	title={Anti-jamming games in multi-channel cognitive radio networks},
	author={Wu, Yongle and Wang, Beibei and Liu, KJ Ray and Clancy, T Charles},
	journal={IEEE journal on selected areas in communications},
	volume={30},
	number={1},
	pages={4--15},
	year={2011},
	publisher={IEEE}
}

@inproceedings{el2014power,
	title={Power control with jammer location uncertainty: A game theoretic perspective},
	author={El-Bardan, Raghed and Brahma, Swastik and Varshney, Pramod K},
	booktitle={2014 48th Annual Conference on Information Sciences and Systems (CISS)},
	pages={1--6},
	year={2014},
	organization={IEEE}
}

@article{cagalj2006wormhole,
	title={Wormhole-based antijamming techniques in sensor networks},
	author={Cagalj, Mario and Capkun, Srdjan and Hubaux, Jean-Pierre},
	journal={IEEE transactions on Mobile Computing},
	volume={6},
	number={1},
	pages={100--114},
	year={2006},
	publisher={IEEE}
}

@article{wang2011anti,
	title={An anti-jamming stochastic game for cognitive radio networks},
	author={Wang, Beibei and Wu, Yongle and Liu, KJ Ray and Clancy, T Charles},
	journal={IEEE journal on selected areas in communications},
	volume={29},
	number={4},
	pages={877--889},
	year={2011},
	publisher={IEEE}
}

@INPROCEEDINGS{8417695, author={Y. {Chen} and Y. {Li} and D. {Xu} and L. {Xiao}}, booktitle={2018 IEEE 87th Vehicular Technology Conference (VTC Spring)}, title={DQN-Based Power Control for IoT Transmission against Jamming}, year={2018}, volume={}, number={}, pages={1-5},}

@INPROCEEDINGS{7952524, author={G. {Han} and L. {Xiao} and H. V. {Poor}}, booktitle={2017 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP)}, title={Two-dimensional anti-jamming communication based on deep reinforcement learning}, year={2017}, volume={}, number={}, pages={2087-2091},}

@article{xiao2018anti,
	title={Anti-jamming underwater transmission with mobility and learning},
	author={Xiao, Liang and Wan, Xiaoyue and Su, Wei and Tang, Yuliang and others},
	journal={IEEE Communications Letters},
	volume={22},
	number={3},
	pages={542--545},
	year={2018},
	publisher={IEEE}
}

@article{khan2017cognitive,
	title={Cognitive-radio-based internet of things: Applications, architectures, spectrum related functionalities, and future research directions},
	author={Khan, Athar Ali and Rehmani, Mubashir Husain and Rachedi, Abderrezak},
	journal={IEEE wireless communications},
	volume={24},
	number={3},
	pages={17--25},
	year={2017},
	publisher={IEEE}
}

@ARTICLE{8314744, author={X. {Liu} and Y. {Xu} and L. {Jia} and Q. {Wu} and A. {Anpalagan}}, journal={IEEE Communications Letters}, title={Anti-Jamming Communications Using Spectrum Waterfall: A Deep Reinforcement Learning Approach}, year={2018}, volume={22}, number={5}, pages={998-1001},}

@article{li2019performance,
	title={On the performance of deep reinforcement learning-based anti-jamming method confronting intelligent jammer},
	author={Li, Yangyang and Wang, Ximing and Liu, Dianxiong and Guo, Qiuju and Liu, Xin and Zhang, Jie and Xu, Yitao},
	journal={Applied Sciences},
	volume={9},
	number={7},
	pages={1361},
	year={2019},
	publisher={Multidisciplinary Digital Publishing Institute}
}

@ARTICLE{6523802, author={R. D. {Pietro} and G. {Oligeri}}, journal={IEEE Network}, title={Jamming mitigation in cognitive radio networks}, year={2013}, volume={27}, number={3}, pages={10-15},}

@inproceedings{wang2011anti,
	title={Anti-jamming communication in cognitive radio networks with unknown channel statistics},
	author={Wang, Qian and Ren, Kui and Ning, Peng},
	booktitle={2011 19th IEEE International Conference on Network Protocols},
	pages={393--402},
	year={2011},
	organization={IEEE}
}

@ARTICLE{8320276, author={H. A. {Bany Salameh} and S. {Almajali} and M. {Ayyash} and H. {Elgala}}, journal={IEEE Internet of Things Journal}, title={Spectrum Assignment in Cognitive Radio Networks for Internet-of-Things Delay-Sensitive Applications Under Jamming Attacks}, year={2018}, volume={5}, number={3}, pages={1904-1913},}

@inproceedings{heo2017dodge,
	title={Dodge-jam: Anti-jamming technique for low-power and lossy wireless networks},
	author={Heo, Jeongyoon and Kim, Jung-Jun and Bahk, Saewoong and Paek, Jeongyeup},
	booktitle={2017 14th Annual IEEE International Conference on Sensing, Communication, and Networking (SECON)},
	pages={1--9},
	year={2017},
	organization={IEEE}
}

@article{kim2015cognitive,
	title={Cognitive Radio Anti-Jamming Scheme for Security Provisioning IoT Communications.},
	author={Kim, Sungwook},
	journal={KSII Transactions on Internet \& Information Systems},
	volume={9},
	number={10},
	year={2015}
}

@inproceedings{rawat2015securing,
	title={Securing space communication systems against reactive cognitive jammer},
	author={Rawat, Danda B and Song, Min},
	booktitle={2015 IEEE Wireless Communications and Networking Conference (WCNC)},
	pages={1428--1433},
	year={2015},
	organization={IEEE}
}

@article{djuraev2017channel,
	title={Channel hopping scheme to mitigate jamming attacks in wireless LANs},
	author={Djuraev, Sirojiddin and Choi, Jin-Ghoo and Sohn, Kyu-Seek and Nam, Seung Yeob},
	journal={EURASIP Journal on Wireless Communications and Networking},
	volume={2017},
	number={1},
	pages={11},
	year={2017},
	publisher={SpringerOpen}
}

@article{becker2014dynamic,
	title={Dynamic beamforming optimization for anti-jamming and hardware fault recovery},
	author={Becker, Jonathan},
	year={2014}
}

@INPROCEEDINGS{7636793, author={S. {Machuzak} and S. K. {Jayaweera}}, booktitle={2016 IEEE/CIC International Conference on Communications in China (ICCC)}, title={Reinforcement learning based anti-jamming with wideband autonomous cognitive radios}, year={2016}, volume={}, number={}, pages={1-5},}

@article{bkassiny2012wideband,
	title={Wideband spectrum sensing and non-parametric signal classification for autonomous self-learning cognitive radios},
	author={Bkassiny, Mario and Jayaweera, Sudharman K and Li, Yang and Avery, Keith A},
	journal={IEEE Transactions on Wireless Communications},
	volume={11},
	number={7},
	pages={2596--2605},
	year={2012},
	publisher={IEEE}
}

@INPROCEEDINGS{7925694, author={M. A. {Aref} and S. K. {Jayaweera} and S. {Machuzak}}, booktitle={2017 IEEE Wireless Communications and Networking Conference (WCNC)}, title={Multi-Agent Reinforcement Learning Based Cognitive Anti-Jamming}, year={2017}, volume={}, number={}, pages={1-6},}

@article{babu2010comprehensive,
	title={A comprehensive analysis of spoofing},
	author={Babu, P Ramesh and Bhaskari, D Lalitha and Satyanarayana, CH},
	journal={International Journal of Advanced Computer Science and Applications},
	volume={1},
	number={6},
	pages={157--62},
	year={2010}
}

@article{whalen2001introduction,
	title={An introduction to arp spoofing},
	author={Whalen, Sean},
	journal={Node99 [Online Document], April},
	year={2001}
}

@ARTICLE{4358709, author={Z. {Duan} and X. {Yuan} and J. {Chandrashekar}}, journal={IEEE Transactions on Dependable and Secure Computing}, title={Controlling IP Spoofing through Interdomain Packet Filters}, year={2008}, volume={5}, number={1}, pages={22-36},}

@INPROCEEDINGS{7804660, author={M. {Nawir} and A. {Amir} and N. {Yaakob} and O. B. {Lynn}}, booktitle={2016 3rd International Conference on Electronic Design (ICED)}, title={Internet of Things (IoT): Taxonomy of security attacks}, year={2016}, volume={}, number={}, pages={321-326},}


@INPROCEEDINGS{7417078, author={L. {Xiao} and Y. {Li} and G. {Liu} and Q. {Li} and W. {Zhuang}}, booktitle={2015 IEEE Global Communications Conference (GLOBECOM)}, title={Spoofing Detection with Reinforcement Learning in Wireless Networks}, year={2015}, volume={}, number={}, pages={1-5},}

@article{liu2017active,
	title={Active authentication with reinforcement learning based on ambient radio signals},
	author={Liu, Jinliang and Xiao, Liang and Liu, Guolong and Zhao, Yifeng},
	journal={Multimedia Tools and Applications},
	volume={76},
	number={3},
	pages={3979--3998},
	year={2017},
	publisher={Springer}
}

@inproceedings{liu2011robust,
	title={Robust physical layer authentication using inherent properties of channel impulse response},
	author={Liu, Fiona Jiazi and Wang, Xianbin and Tang, Helen},
	booktitle={2011-MILCOM 2011 Military Communications Conference},
	pages={538--542},
	year={2011},
	organization={IEEE}
}

@ARTICLE{7398138, author={L. {Xiao} and Y. {Li} and G. {Han} and G. {Liu} and W. {Zhuang}}, journal={IEEE Transactions on Vehicular Technology}, title={PHY-Layer Spoofing Detection With Reinforcement Learning in Wireless Networks}, year={2016}, volume={65}, number={12}, pages={10037-10047},}

@incollection{xiao2019learning,
	title={Learning-Based Rogue Edge Detection in VANETs with Ambient Radio Signals},
	author={Xiao, Liang and Zhuang, Weihua and Zhou, Sheng and Chen, Cailian},
	booktitle={Learning-based VANET Communication and Security Techniques},
	pages={13--47},
	year={2019},
	publisher={Springer}
}

@INPROCEEDINGS{8046382, author={E. {Yel} and T. X. {Lin} and N. {Bezzo}}, booktitle={2017 NASA/ESA Conference on Adaptive Hardware and Systems (AHS)}, title={Reachability-based self-triggered scheduling and replanning of UAV operations}, year={2017}, volume={}, number={}, pages={221-228},}

@inproceedings{bezzo2018predicting,
	title={Predicting malicious intention in CPS under cyber-attack},
	author={Bezzo, Nicola},
	booktitle={2018 ACM/IEEE 9th International Conference on Cyber-Physical Systems (ICCPS)},
	pages={351--352},
	year={2018},
	organization={IEEE}
}

@inproceedings{ramachandran2007bayesian,
	title={Bayesian Inverse Reinforcement Learning.},
	author={Ramachandran, Deepak and Amir, Eyal},
	booktitle={IJCAI},
	volume={7},
	pages={2586--2591},
	year={2007}
}

@inproceedings{elnaggar2018irl,
	title={An IRL approach for cyber-physical attack intention prediction and recovery},
	author={Elnaggar, Mahmoud and Bezzo, Nicola},
	booktitle={2018 Annual American Control Conference (ACC)},
	pages={222--227},
	year={2018},
	organization={IEEE}
}

@article{yan2016q,
	title={Q-learning-based vulnerability analysis of smart grid against sequential topology attacks},
	author={Yan, Jun and He, Haibo and Zhong, Xiangnan and Tang, Yufei},
	journal={IEEE Transactions on Information Forensics and Security},
	volume={12},
	number={1},
	pages={200--210},
	year={2016},
	publisher={IEEE}
}



@article{chen2018evaluation,
	title={Evaluation of reinforcement learning-based false data injection attack to automatic voltage control},
	author={Chen, Ying and Huang, Shaowei and Liu, Feng and Wang, Zhisheng and Sun, Xinwei},
	journal={IEEE Transactions on Smart Grid},
	volume={10},
	number={2},
	pages={2158--2169},
	year={2018},
	publisher={IEEE}
}

@ARTICLE{8514804, author={M. N. {Kurt} and O. {Ogundijo} and C. {Li} and X. {Wang}}, journal={IEEE Transactions on Smart Grid}, title={Online Cyber-Attack Detection in Smart Grid: A Reinforcement Learning Approach}, year={2019}, volume={10}, number={5}, pages={5174-5185},}

@inproceedings{wang2013survey,
	title={A survey on bad data injection attack in smart grid},
	author={Wang, Dai and Guan, Xiaohong and Liu, Ting and Gu, Yun and Sun, Yanan and Liu, Yang},
	booktitle={2013 IEEE PES Asia-Pacific Power and Energy Engineering Conference (APPEEC)},
	pages={1--6},
	year={2013},
	organization={IEEE}
}

@ARTICLE{8603817, author={Z. {Ni} and S. {Paul}}, journal={IEEE Transactions on Neural Networks and Learning Systems}, title={A Multistage Game in Smart Grid Security: A Reinforcement Learning Solution}, year={2019}, volume={30}, number={9}, pages={2684-2695},}


@techreport{pillitteri2014guidelines,
	title={Guidelines for smart grid cybersecurity},
	author={Pillitteri, Victoria Y and Brewer, Tanya L},
	year={2014}
}

@inproceedings{zhu2014sequential,
	title={The sequential attack against power grid networks},
	author={Zhu, Yihai and Yan, Jun and Tang, Yufei and Sun, Yan and He, Haibo},
	booktitle={2014 IEEE International Conference on Communications (ICC)},
	pages={616--621},
	year={2014},
	organization={IEEE}
}


@inproceedings{loch1998using,
	title={Using Eligibility Traces to Find the Best Memoryless Policy in Partially Observable Markov Decision Processes.},
	author={Loch, John and Singh, Satinder P},
	booktitle={ICML},
	pages={323--331},
	year={1998}
}

@online{woolf,
	author = {Woolf, Nicky},
	title  = {DDoS attack that disrupted internet was largest of its kind in history, experts say},
	date   = {2016-10},
	url    = {https://www.theguardian.com/technology/2016/oct/26/ddos-attack-dyn-mirai-botnet}
}

@inproceedings{antonakakis2017understanding,
	title={Understanding the mirai botnet},
	author={Antonakakis, Manos and April, Tim and Bailey, Michael and Bernhard, Matt and Bursztein, Elie and Cochran, Jaime and Durumeric, Zakir and Halderman, J Alex and Invernizzi, Luca and Kallitsis, Michalis and others},
	booktitle={26th $\{$USENIX$\}$ Security Symposium ($\{$USENIX$\}$ Security 17)},
	pages={1093--1110},
	year={2017}
}

@ARTICLE{8231220, author={L. {Xiao} and C. {Xie} and M. {Min} and W. {Zhuang}}, journal={IEEE Transactions on Vehicular Technology}, title={User-Centric View of Unmanned Aerial Vehicle Transmission Against Smart Attacks}, year={2018}, volume={67}, number={4}, pages={3420-3430},}

@inproceedings{lu2017anti,
	title={Anti-jamming communication game for UAV-aided VANETs},
	author={Lu, Xiaozhen and Xu, Dongjin and Xiao, Liang and Wang, Lei and Zhuang, Weihua},
	booktitle={GLOBECOM 2017-2017 IEEE Global Communications Conference},
	pages={1--6},
	year={2017},
	organization={IEEE}
}

@ARTICLE{8246580, author={L. {Xiao} and X. {Lu} and D. {Xu} and Y. {Tang} and L. {Wang} and W. {Zhuang}}, journal={IEEE Transactions on Vehicular Technology}, title={UAV Relay in VANETs Against Smart Jamming With Reinforcement Learning}, year={2018}, volume={67}, number={5}, pages={4087-4097},}

@INPROCEEDINGS{8761101, author={S. {Feng} and S. {Haykin}}, booktitle={ICC 2019 - 2019 IEEE International Conference on Communications (ICC)}, title={Anti-Jamming V2V Communication in an Integrated UAV-CAV Network with Hybrid Attackers}, year={2019}, volume={}, number={}, pages={1-6},}

@INPROCEEDINGS{8417685, author={M. {Min} and L. {Xiao} and D. {Xu} and L. {Huang} and M. {Peng}}, booktitle={2018 IEEE 87th Vehicular Technology Conference (VTC Spring)}, title={Learning-Based Defense against Malicious Unmanned Aerial Vehicles}, year={2018}, volume={}, number={}, pages={1-5},}

@ARTICLE{8727523, author={M. {Zhang} and C. {Dong} and Y. {Huang}}, journal={IEEE Access}, title={FS-MAC: An Adaptive MAC Protocol With Fault-Tolerant Synchronous Switching for FANETs}, year={2019}, volume={7}, number={}, pages={80602-80613},}

@INPROCEEDINGS{8855737, author={N. {Alsaffar} and H. {Ali} and W. {Elmedany}}, booktitle={2018 International Conference on Innovation and Intelligence for Informatics, Computing, and Technologies (3ICT)}, title={Smart Transportation System: A Review of Security and Privacy Issues}, year={2018}, volume={}, number={}, pages={1-4},}

@article{javed2016security,
	title={Security in intelligent transport systems for smart cities: From theory to practice},
	author={Javed, Muhammad Awais and Ben Hamida, Elyes and Znaidi, Wassim},
	journal={Sensors},
	volume={16},
	number={6},
	pages={879},
	year={2016},
	publisher={Multidisciplinary Digital Publishing Institute}
}

@article{karagiannis2011vehicular,
	title={Vehicular networking: A survey and tutorial on requirements, architectures, challenges, standards and solutions},
	author={Karagiannis, Georgios and Altintas, Onur and Ekici, Eylem and Heijenk, Geert and Jarupan, Boangoat and Lin, Kenneth and Weil, Timothy},
	journal={IEEE communications surveys \& tutorials},
	volume={13},
	number={4},
	pages={584--616},
	year={2011},
	publisher={IEEE}
}

@article{auer2002finite,
	title={Finite-time analysis of the multiarmed bandit problem},
	author={Auer, Peter and Cesa-Bianchi, Nicolo and Fischer, Paul},
	journal={Machine learning},
	volume={47},
	number={2-3},
	pages={235--256},
	year={2002},
	publisher={Springer}
}

@article{weng2018bandit,
	title   = "The Multi-Armed Bandit Problem and Its Solutions",
	author  = "Weng, Lilian",
	journal = "lilianweng.github.io/lil-log",
	year    = "2018",
	url     = "http://lilianweng.github.io/lil-log/2018/01/23/the-multi-armed-bandit-problem-and-its-solutions.html"
}

@inproceedings{lazaric2008reinforcement,
	title={Reinforcement learning in continuous action spaces through sequential monte carlo methods},
	author={Lazaric, Alessandro and Restelli, Marcello and Bonarini, Andrea},
	booktitle={Advances in neural information processing systems},
	pages={833--840},
	year={2008}
}

@inproceedings{kulkarni2016hierarchical,
	title={Hierarchical deep reinforcement learning: Integrating temporal abstraction and intrinsic motivation},
	author={Kulkarni, Tejas D and Narasimhan, Karthik and Saeedi, Ardavan and Tenenbaum, Josh},
	booktitle={Advances in neural information processing systems},
	pages={3675--3683},
	year={2016}
}
